ELBA: Learning by Asking for Embodied Visual Navigation and Task Completion

The research community has shown increasing interest in designing intelligent embodied agents that can assist humans in accomplishing tasks. Although there have been significant advancements in related vision-language benchmarks, most prior work has focused on building agents that follow instructions rather than endowing agents the ability to ask questions to actively resolve ambiguities arising naturally in embodied environments. To address this gap, we propose an Embodied Learning-By-Asking (ELBA) model that learns when and what questions to ask to dynamically acquire additional information for completing the task. We evaluate ELBA on the TEACh vision-dialog navigation and task completion dataset. Experimental results show that the proposed method achieves improved task performance compared to baseline models without question-answering capabilities.

==> sections/8_limitations.tex <==
\section{Limitations}
We also observe a few notable limitations. One major challenge is the quality of the QA Evaluator. The QA Evaluator cannot distinguish between confusing QA pairs and reasonable QA pairs. One possible cause is that, although our approach presents a viable way to generate different types of question-and-answer pairs, the within-domain training dataset for the QA Evaluator is not large enough. Another problem is that we use all the future sub-goals predicted by the \textsc{Planner} as candidate answers rather than constructing candidate answers from the next sub-goal instruction only. The latter approach requires the model to track the completion status of the current sub-goal so that the model can decide when to ask questions about the next sub-goal. However, our current model cannot track the status of sub-goal completion; therefore, we let the model treat all future sub-goals as candidate answers. This helps avoid the problem of tracking sub-goal status, but it also leads to ill-timed questions during inference. 

